Many Body Symmetrical Dynamical Systems

We investigate the stability of few body symmetrical dynamical systems which include four and five body symmetrical dynamical systems. Research presented in this thesis includes the following original investigations: determination of some analytical solutions of the four body problem; stability analysis of the near symmetric coplanar CSFBP ; derivation of the analytical stability criterion valid for all time for a special symmetric configuration of the general five-body problem, the CS5BP, which exhibits many of the salient characteristics of the general five body problem; numerical investigation of the hierarchical stability of the CS5BP and derivation of the stability criterion for the CSNBP.

==> LinearStabiliyanalysis.tex <==

\chapter{Linear Stability Analysis of the Four-Body equilibrium solutions}

In Chapter 3 we discussed the equilibrium configurations for
various cases of the four body problem. We will now complete a
linear stability analysis of these solutions.

We first derive the equations of motion for the general four body
problem in a rotating frame of reference in section 4.1. In
section 4.2 we derive the linear stability criterion for the
equilibrium points. This criterion is derived by using the
standard method of Classical Mechanics i.e. by perturbing one of
the particles from its Lagrange point. If the resultant motion of
the particle, after perturbation, is a rapid departure from the
vicinity of the point we can call such a position of equilibrium
an unstable one, but if the particle oscillates about the point it
is said to be a stable position. In section 4.3 we apply our
stability criterion to the equilibrium configurations discussed in
chapter 2. Linear stability of the equal mass cases, have already
been discussed by \citeasnoun{JaganBonnie} which we will revisit
using our own standard method of Celestial Mechanics. We conclude
that all the equal mass cases are unstable which agrees with the
results of \citeasnoun{JaganBonnie}. We also show that any
configuration with a pair of equal masses are unstable. In section
4.4 we give summary of the conclusions of the chapter.

\section{The Equations of motion}

In this section, the equations of motion for the four body problem
are derived in a rotating frame of reference . We consider the
motion of a particle moving under the gravitational influence of
three particles of masses $m_{1}$ , $m_{2}$ and $m_{3}$. Let all
the four particles (masses) have circular orbits about their
common center of mass. Consider a set of axes $\xi ,\eta ,\zeta $
in the inertial frame having its origin at the center of mass of
the system. Let the coordinates of the three masses in this
reference frame be $(\xi _{1},\eta _{1},\zeta _{1})$ , $(\xi
_{2},\eta _{2},\zeta _{2})$ and $(\xi _{3},\eta _{3},\zeta _{3})$.
Let the coordinates of the fourth mass be $(\xi ,\eta ,\zeta )$.
By applying the vector form of the inverse square law, the
equations of motion of the particle are (See any standard text for
details, for example \citeasnoun{CarlMurray})

\begin{equation}
\stackrel{..}{\xi }=m_{1}\frac{\xi _{1}-\xi
}{r_{14}^{3}}+m_{2}\frac{\xi _{2}-\xi }{r_{24}^{3}}+m_{3}\frac{\xi
_{3}-\xi }{r_{34}^{3}},  \label{1.1}
\end{equation}
\begin{equation}
\stackrel{..}{\eta }=m_{1}\frac{\eta _{1}-\eta
}{r_{14}^{3}}+m_{2}\frac{\eta _{2}-\eta
}{r_{24}^{3}}+m_{3}\frac{\eta _{3}-\eta }{r_{34}^{3}},
\label{1.2}
\end{equation}
\begin{equation}
\stackrel{..}{\xi }=m_{1}\frac{\zeta _{1}-\zeta }{r_{14}^{3}}+m_{2}\frac{%
\zeta _{2}-\zeta }{r_{24}^{3}}+m_{3}\frac{\zeta _{3}-\zeta
}{r_{34}^{3}}, \label{1.3}
\end{equation}
where,
\begin{equation}
r_{14}^{2}=(\xi _{1}-\xi )^{2}+(\eta _{1}-\eta )^{2}+(\zeta
_{1}-\zeta )^{2},
\end{equation}
\begin{equation}
r_{24}^{2}=(\xi _{2}-\xi )^{2}+(\eta _{2}-\eta )^{2}+(\zeta
_{2}-\zeta )^{2},
\end{equation}
\begin{equation}
r_{34}^{2}=(\xi _{3}-\xi )^{2}+(\eta _{3}-\eta )^{2}+(\zeta
_{3}-\zeta )^{2}.
\end{equation}


Note that these equations are also valid in the general four-body
problem, since they do not require any assumptions about the paths
of the masses.

The motion of the four masses in circular orbits fixes the
distances between them and they move about their common center of
mass at a fixed angular velocity, the mean motion $n$. In these
circumstances it is natural to consider the motion of the particle
in a rotating reference frame in which the location of the three
masses are also fixed. Consider a new rotating coordinate system
that also has the origin at the center of mass of the system but
which is rotating at a uniform rate $n$ in the positive
direction. The coordinates of the three masses, in our arrangement, are $%
(x_{1},y_{1},0)$, $(x_{2},0,0)$ and $(x_{3},y_{3},0).$ These
coordinates are related to the non-rotating coordinate system by
the simple relation

\begin{equation}
\left(
\begin{array}{c}
\xi \\
\eta \\
\zeta
\end{array}
\right) =\left(
\begin{array}{ccc}
\cos nt & -\sin nt & 0 \\
\sin nt & \cos nt & 0 \\
0 & 0 & 1
\end{array}
\right) \left(
\begin{array}{c}
x \\
y \\
z
\end{array}
\right) .  \label{1.5}
\end{equation}


Differentiating each component in Equation(\ref{1.5}) twice we get

\begin{equation}
\left(
\begin{array}{c}
\stackrel{..}{\xi } \\
\stackrel{..}{\eta } \\
\stackrel{..}{\zeta }
\end{array}
\right) =\left(
\begin{array}{ccc}
\cos nt & -\sin nt & 0 \\
\sin nt & \cos nt & 0 \\
0 & 0 & 1
\end{array}
\right) \left(
\begin{array}{c}
\stackrel{..}{x}-2n\stackrel{.}{y}-n^{2}x \\
\stackrel{..}{y}+2n\stackrel{.}{x}-n^{2}y \\
\stackrel{..}{z}
\end{array}
\right) .
\end{equation}
The coordinate transformation from a non-rotating reference frame
to a rotating frame has introduced terms in $n\stackrel{.}{x}$ and
$n\stackrel{.}{ y}$ ( {\it The Corioli's acceleration}) and
$n^{2}x$ and $n^{2}y$ ({\it the centrifugal acceleration}) into
the equations of motion. Substituting $\xi ,\eta ,\zeta $ and its
derivatives into Equation (\ref{1.1}), (\ref{1.2}) and (
\ref{1.3}) we get
\begin{eqnarray}
&&(\stackrel{..}{x}-2n\stackrel{.}{y}-n^{2}x)\cos nt-(\stackrel{..}{y}+2n%
\stackrel{.}{x}-n^{2}y)\sin nt=  \nonumber \\
&&(m_{1}\frac{x_{1}-x}{r_{14}^{3}}+m_{2}\frac{x_{2}-x}{r_{24}^{3}}+m_{3}%
\frac{x_{3}-x}{r_{34}^{3}})\cos nt  \label{1.6} \\
&&+(m_{1}\frac{y_{1}-y}{r_{14}^{3}}+m_{2}\frac{y_{2}-y}{r_{24}^{3}}+m_{3}%
\frac{y_{3}-y}{r_{34}^{3}})\sin nt,  \nonumber
\end{eqnarray}
\begin{eqnarray}
&&(\stackrel{..}{x}-2n\stackrel{.}{y}-n^{2}x)\sin nt+(\stackrel{..}{y}+2n%
\stackrel{.}{x}-n^{2}y)\cos nt=  \nonumber \\
&&(m_{1}\frac{x_{1}-x}{r_{14}^{3}}+m_{2}\frac{x_{2}-x}{r_{24}^{3}}+m_{3}%
\frac{x_{3}-x}{r_{34}^{3}})\sin nt  \label{1.7} \\
&&+(m_{1}\frac{y_{1}-y}{r_{14}^{3}}+m_{2}\frac{y_{2}-y}{r_{24}^{3}}+m_{3}%
\frac{y_{3}-y}{r_{34}^{3}})\cos nt,  \nonumber
\end{eqnarray}
\begin{equation}
\stackrel{..}{z}=-(\frac{m_{1}}{r_{14}^{3}}+\frac{m_{2}}{r_{24}^{3}}+\frac{%
m_{3}}{r_{34}^{3}})z.  \label{1.8}
\end{equation}
where
\begin{equation}
r_{14}^{2}=(x-x_{1})^{2}+(y-y_{1})^{2}+z^{2}
\end{equation}
\begin{equation}
r_{24}^{2}=(x-x_{2})^{2}+(y-y_{2})^{2}+z^{2}
\end{equation}
\begin{equation}
r_{34}^{2}=(x-x_{3})^{2}+(y-y_{3})^{2}+z^{2}
\end{equation}
If we multiply Equation(\ref{1.6}) by $\cos nt$, and
Equation(\ref{1.7}) by $\sin nt,$ and add the results, and then
multiply Equation (\ref{1.6}) by $-\sin nt$, and Equation(
\ref{1.7}) by $\cos nt$ and add these together, the equations of
motion in the rotating coordinate system become
\begin{equation}
(\stackrel{..}{x}-2n\stackrel{.}{y}-n^{2}x)=(m_{1}\frac{x_{1}-x}{r_{14}^{3}}
+m_{2}\frac{x_{2}-x}{r_{24}^{3}}+m_{3}\frac{x_{3}-x}{r_{34}^{3}}),
\label{1.17}
\end{equation}
\begin{equation}
(\stackrel{..}{y}+2n\stackrel{.}{x}-n^{2}y)=(m_{1}\frac{y_{1}-y}{r_{14}^{3}}%
+m_{2}\frac{y_{2}-y}{r_{24}^{3}}+m_{3}\frac{y_{3}-y}{r_{34}^{3}}),
\label{1.18}
\end{equation}
\begin{equation}
\stackrel{..}{z}=-(\frac{m_{1}}{r_{14}^{3}}+\frac{m_{2}}{r_{24}^{3}}+\frac{%
m_{3}}{r_{34}^{3}})z.  \label{1.19}
\end{equation}
Let a function $U=U(x,y,z)$ be defined by
\begin{equation}
U=\frac{n^{2}}{2}(x^{2}+y^{2})+\frac{m_{1}}{r_{14}}+\frac{m_{2}}{r_{24}}+%
\frac{m_{3}}{r_{34}}
\end{equation}
then it can easily be seen that Equations (\ref{1.17}),
(\ref{1.18}) and (\ref {1.19}) may be written as
\begin{equation}
\stackrel{..}{x}-2n\stackrel{.}{y}=\frac{\partial U}{\partial x},
\label{1.9}
\end{equation}
\begin{equation}
\stackrel{..}{y}+2n\stackrel{.}{x}=\frac{\partial U}{\partial y},
\label{1.10}
\end{equation}
\begin{equation}
\stackrel{..}{z}=\frac{\partial U}{\partial z},  \label{1.11}
\end{equation}

\section{Stability Criterion for the Equilibrium Points}

In chapter 3 we have found Equilibrium points for different
geometrical arrangements for the four body problem. We now would
like to determine the stability of such points. In this section a
standard procedure for determining linear stability will be
developed. To do this we extend the method as given by
\citeasnoun{CarlMurray} for the three body problem, to the four
body problem. The procedure will then be applied to the following
special solutions of the four body problem to determine their
stability:

\begin{enumerate}
\item  All Equal mass cases.

\item  All cases with two pairs of equal masses.
\end{enumerate}

In order to carry out a proper study of the stability we need to
examine the behavior of a particle that is given a small
displacement from an equilibrium position. We will follow the well
known linearization procedure for linearizing the equations of
motion and carrying out a  linear stability analysis (see any
standard text for further details).

As all the equilibrium solutions of chapter 3 are coplanar, we
will use the coplanar equations from now on in this chapter. Let
the location of an equilibrium point in the circular four-body
problem be denoted by $(x_{0},y_{0})$ and consider a small
displacement $(X,Y)$ from the point such that $x=x_{0}+X$ and
$y=y_{0}+Y$. Then by substituting in Equations (\ref{1.9}) and
(\ref{1.10}), and expanding in Taylor series, we have
\begin{eqnarray}
\stackrel{..}{X}-2n\stackrel{.}{Y} &\approx &\left( \frac{\partial U}{%
\partial x}\right) _{0}+X\left( \frac{\partial }{\partial x}\left( \frac{%
\partial U}{\partial x}\right) \right) _{0}+Y\left( \frac{\partial }{
\partial y}\left( \frac{\partial U}{\partial x}\right) \right) _{0}+\cdots
\nonumber \\
&=&X\left( \frac{\partial ^{2}U}{\partial x^{2}}\right)
_{0}+Y\left( \frac{
\partial ^{2}U}{\partial x\partial y}\right) _{0}+\cdots ,
\end{eqnarray}
and
\[
\stackrel{..}{Y}+2n\stackrel{.}{X\approx \left( \frac{\partial
U}{\partial y} \right) _{0}+X}\left( \frac{\partial }{\partial
x}\left( \frac{\partial U}{
\partial y}\right) \right) _{0}+Y\left( \frac{\partial }{\partial y}\left(
\frac{\partial U}{\partial y}\right) \right) _{0}+\cdots
\]
\begin{equation}
=X\left( \frac{\partial ^{2}U}{\partial x\partial y}\right)
_{0}+Y\left( \frac{\partial ^{2}U}{\partial y\partial ^{2}}\right)
_{0}+\cdots \textrm{,\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }
\end{equation}
where the suffix zero means that after the partial derivatives of
$U$ are accomplished $x,\,y\,$and $z$ are set equal to
$x_{0},y_{0}$ and $z_{0}$
respectively. We have used the fact that $\left( \frac{\partial U}{\partial x%
}\right) _{0}=\left( \frac{\partial U}{\partial y}\right) _{0}=0$
(because the equilibrium points are derived by solving the
equations $\partial U/\partial x=\partial U/\partial y=0)$.
Because of our interest in the motion in the immediate vicinity of
the equilibrium points, the higher order terms are neglected.
These higher order terms will always be small quantities. Carrying
out the standard procedure to {\it linearize }the equations of
motion, the end result is a set of linear differential equations
of the form
\begin{equation}
\stackrel{..}{X}-2\stackrel{.}{Y}=XU_{xx}+YU_{xy},
\end{equation}
\begin{equation}
\stackrel{..}{Y}+2\stackrel{.}{X}=XU_{xy}+YU_{yy},
\end{equation}
where we have taken $n=1$ and the quantities
\begin{equation}
Uxx=\left( \frac{\partial ^{2}U}{\partial x^{2}}\right)
_{0}\textrm{ etc.}
\end{equation}

and the $U$ are all constants since they are evaluated at
equilibrium point.

The linearized equations in the matrix form are
\begin{equation}
\left(
\begin{array}{c}
\stackrel{.}{X} \\
\stackrel{.}{Y} \\
\stackrel{..}{X} \\
\stackrel{..}{Y}
\end{array}
\right) =\left(
\begin{array}{cccc}
0 & 0 & 1 & 0 \\
0 & 0 & 0 & 1 \\
U_{xx} & U_{xy} & 0 & 2 \\
U_{xy} & U_{yy} & -2 & 0
\end{array}
\right) \left(
\begin{array}{c}
X \\
Y \\
\stackrel{.}{X} \\
\stackrel{.}{Y}
\end{array}
\right) ,
\end{equation}
Our problem of solving two simultaneous second order differential
equations is changed to solving four, simultaneous, first order
differential equations. These equations can also be written in the
following matrix form
\begin{equation}
\stackrel{.}{{\bf X}}={\bf AX,}  \label{1.12}
\end{equation}
where
\begin{equation}
{\bf X=}\left(
\begin{array}{c}
\stackrel{.}{X} \\
\stackrel{.}{Y} \\
\stackrel{..}{X} \\
\stackrel{..}{Y}
\end{array}
\right) \textrm{ and }{\bf A=}\left(
\begin{array}{cccc}
0 & 0 & 1 & 0 \\
0 & 0 & 0 & 1 \\
U_{xx} & U_{xy} & 0 & 2 \\
U_{xy} & U_{yy} & -2 & 0
\end{array}
\right) .
\end{equation}

If any vector {\bf X }satisfies the equation
\begin{equation}
\bf AX=\lambda X, \label{1.13}
\end{equation}
where $\lambda $ is a scalar constant, then {\bf X} is said to be
an {\it eigenvector} of the matrix {\bf A} and $\lambda $ is the
corresponding  eigenvalue.

The first step in the solution of Equation (\ref{1.12}) is to find
the eigenvalues of {\bf A. }We can rewrite Equation (\ref{1.13})
as
\begin{equation}
\left( {\bf A}-\lambda {\bf I}\right) {\bf X=0,}
\end{equation}
where I is a $4\times 4$\ unit matrix. The characteristic equation
is given by
\begin{equation}
\det ({\bf A-\lambda I)=}\left|
\begin{array}{cccc}
-\lambda & 0 & 1 & 0 \\
0 & -\lambda & 0 & 1 \\
U_{xx} & U_{xy} & -\lambda & 2 \\
U_{xy} & U_{yy} & -2 & -\lambda
\end{array}
\right| =0
\end{equation}
which reduces to the polynomial equation
\begin{equation}
\lambda ^{4}+\left( 4-U_{xx}-U_{yy}\right) \lambda
^{2}+U_{xx}U_{yy}-U_{xy}^{2}=0.  \label{1.14}
\end{equation}
Equation (\ref{1.14}) is a quartic equation in the variable
$\lambda $ but it is also quadratic in $\lambda ^{2}$. This makes
it relatively easy to find the four roots. They are
\begin{equation}
\lambda _{1,2}=\pm \left[ \frac{1}{2}\left( U_{xx}+U_{yy}-4\right) -\frac{1}{%
2}\left[ \left( 4-U_{xx}-U_{yy}\right) ^{2}-4\left(
U_{xx}U_{yy}-U_{xy}^{2}\right) \right] ^{1/2}\right] ^{1/2}
\label{1.15}
\end{equation}
and
\begin{equation}
\lambda _{3,4}=\pm \left[ \frac{1}{2}\left( U_{xx}+U_{yy}-4\right)
+\frac{1}{ 2}\left[ \left( 4-U_{xx}-U_{yy}\right) ^{2}-4\left(
U_{xx}U_{yy}-U_{xy}^{2}\right) \right] ^{1/2}\right] ^{1/2}
\label{1.16}
\end{equation}

 The stability of the equilibrium points can be determined from an
analysis of the eigenvalues alone. To investigate the nature of
eigenvalues we define the quantities
\begin{eqnarray}
A&=&\frac{m_{1}}{r_{1}^{3}}+\frac{m_{2}}{r_{2}^{3}}+\frac{m_{3}}{r_{3}^{3}},\\
%\end{equation}
%\begin{equation}
B&=&3\left[ m_{1}\frac{\left( y-y_{1}\right)
^{2}}{r_{1}^{5}}+m_{2}\frac{ \left( y-y_{2}\right)
^{2}}{r_{2}^{5}}+m_{3}\frac{\left( y-y_{3}\right) ^{2}
}{r_{3}^{5}}\right] ,\\ \nonumber
%\end{equation}
%\begin{equation}
C&=&3\left[ m_{1}\frac{\left( x-x_{1}\right) \left( y-y_{1}\right)
}{r_{1}^{5}} +m_{2}\frac{\left( x-x_{2}\right) \left(
y-y_{2}\right) }{r_{2}^{5}}+m_{3} \frac{\left( x-x_{3}\right)
\left( y-y_{3}\right) }{r_{3}^{5}}\right] ,\\ \\
%\end{equation}
%\begin{equation}
D&=&3\left[ m_{1}\frac{\left( x-x_{1}\right)
^{2}}{r_{1}^{5}}+m_{2}\frac{ \left( x-x_{2}\right)
^{2}}{r_{2}^{5}}+m_{3}\frac{\left( x-x_{3}\right) ^{2}
}{r_{3}^{5}}\right] .
\end{eqnarray}
In terms of $A,B,C$ and $D$ we can write
\begin{equation}
U_{xx}=1-A+D,
\end{equation}
\begin{equation}
U_{yy}=1-A+B,
\end{equation}
\begin{equation}
U_{xy}=C.
\end{equation}

The general form of the eigenvalues given in (\ref{1.16}) is
\begin{equation}
\lambda _{1,2}=\pm \left( j_{1}+ik_{1}\right) ,\qquad \lambda
_{3,4}=\pm \left( j_{2}+ik_{2}\right) ,
\end{equation}

If the eigenvalues are pure imaginary numbers, then an oscillatory
solution will result because terms with $e^{\pm ikt}$ will reduce
to sines and cosines. However, if its real part is non-zero then
there will always be exponential growth in at least one mode and
so the perturbed solution will be unstable. Therefore the
equilibrium point will be stable if all the eigenvalues are purely
imaginary. We will apply this analysis to special cases of four
body problem of equal masses and with two pairs of equal masses.
\section{Linear Stability analysis of the equilibrium points}
\subsection{Equilibrium Configuration of four body problem with four equal
masses making a square}

Here we consider the four body problem of four equal masses making
a square \cite{RoyandSteves1998}. \citeasnoun{JaganBonnie} have
discussed its stability and shown that this configuration is
unstable. Now we will also discuss its stability as a test case
for our method developed at the beginning of this section.

In this highly symmetric case of the four body problem we consider
the origin of the coordinate system to be at the centre of mass
and therefore all four bodies are equally spaced on the axis. i.e.
\begin{equation}
r_{1}=r_{2}=r_{3}=a\textrm{ and }r_{14}=r_{34}.
\end{equation}
Using all the relevant available information we get
\begin{eqnarray}
Uxx&=&1 + \frac{0.0159}{a^3}\\
Uxy&=&1 +\frac{ 0.5519}{a^3}\\
\textrm{ and }Uyy&=&\frac{0.422}{a^3}
\end{eqnarray}
Hence from equations (\ref{1.15}) and (\ref{1.16}) we get the
following eigenvalues
\begin{eqnarray}
\lambda_{1,2}=\pm
\frac{1}{2}\sqrt{-4+\frac{1.136}{a^3}-2\sqrt{\frac{1.003}{a^6}-\frac{4.544}{a^3}}}\\
\lambda_{3,4}=\pm
\frac{1}{2}\sqrt{-4+\frac{1.136}{a^3}+2\sqrt{\frac{1.003}{a^6}-\frac{4.544}{a^3}}}
\end{eqnarray}
By substituting $n=M=1$ in equation (3.10) we get $a=1.3937$ and
hence the following eigenvalues:
\begin{equation}
\lambda _{1,2}=(-0.311626 \mp 0.996094 i)\textrm{ and }\lambda
_{3,4}=\pm (0.311626 \mp 0.996094 i).
\end{equation}


The real part of all the eigenvalues is not equal to zero.
Therefore there will be an exponential growth in all directions
which shows that this configuration is linearly unstable to
perturbations. This result is in confirmation with the result
obtained by \citeasnoun{JaganBonnie}.

\subsection{Equilateral Triangle equilibrium configuration of four body
equal mass problem}

Consider the equilateral triangle equilibrium configuration of
equal mass four body problem \cite{JaganBonnie}. Let the fourth
mass be at the centre of mass which is also the centroid of the
triangle. \citeasnoun{JaganBonnie} showed that this configuration
is linearly unstable to perturbations. We will again use our
method to check its stability. This will also serve as a test case
for our method.

Consider the centre of mass to be the centroid of the triangle. As
this is an equilateral triangle configuration therefore
\begin{equation}
r_{14}=r_{24}=r_{34}=\frac{a}{\sqrt{3}}\textrm{ and
}r_{13}=r_{23}=r_{12}=a
\end{equation}
This shows that all three bodies are equidistant from the centre
of mass. The initial conditions are
$$
(x,y) =(0,0);\qquad (x_1,y_1) = (\frac{-1}{2a},
\frac{-1}{\sqrt{12}}a);
$$

$$
(x_2,y_2) =(0, \frac{1}{\sqrt{3}}a); (x_3,y_3)=(0.5a,
\frac{-1}{\sqrt{12}}a)
$$

Using the above initial conditions we get

\begin{eqnarray}
Uxx&=&1 - \frac{5.84}{a^2} -\frac{3.897}{a^3},\\
Uxy&=&0\\
Uyy&=&1 + \frac{7.79}{a^3}
\end{eqnarray}

By substituting $n=M=1$ in equation (3.16) we get $a=2.016$. Now
from equations (4.34) and (4.35) we get
\begin{equation}
\lambda _{1,2}=\pm (0.716297)\textrm{ and }\lambda _{3,4}=\pm
(1.86434i).
\end{equation}
As two of the four eigenvalues are real, this configuration is
linearly unstable to perturbations, confirming the results of
\citeasnoun{JaganBonnie}. It is to be noted that $a$ gives the
size of the triangle and therefore does not have any effect on the
form of the eigenvalues and hence the stability of the system.

\subsection{Collinear equilibrium configuration of the equal mass four body
problem.}

Consider the collinear equilibrium configuration of the equal mass
four body problem \cite{RoyandSteves1998}. Its stability has also
been discussed by \citeasnoun{JaganBonnie} using their own method.
We will use our method to discuss its stability. The initial
conditions are
\begin{eqnarray}
\left( x,y\right) &=&\left( -1,0\right)r_1 ,\left( x_{1},y_{1}\right) =(1,0)r_1, \\
\left( x_{2},y_{2}\right) &=&\left( \alpha ,0\right)r_1 \textrm{
and }\left( x_{3},y_{3}\right) =\left( -\alpha ,0\right)r_1 ,
\end{eqnarray}
where $\alpha =0.316$ and hence
\begin{equation}
U_{xx}=1+2A,U_{yy}=1-A\textrm{ and }U_{xy}=0.
\end{equation}
The eigenvalues are
\begin{equation}
\lambda _{1,2}=\pm (1.18218)\textrm{ and }\lambda _{3,4}=\pm
0.811759
\end{equation}
As two of the eigenvalues are real, the configuration is linearly
unstable to perturbations, confirming the results of
\citeasnoun{JaganBonnie}

Now we will determine the stability of equilibrium configurations
of the following cases of two pairs of equal masses.

\subsection{The Triangular equilibrium configuration of the four-body problem with two bigger
masses making the base of the triangle}

We consider the triangular configuration of the four-body problem
having two pairs of equal masses with the fourth mass on the
positive y-axis and the two bigger masses making the base of the
triangle. We have already obtained equilibrium solutions for it in
chapter 2 and now will discuss its stability.

The initial conditions are
\begin{eqnarray}
\left( x,y\right) &=&\left( C_{4}X,0\right)r_{31} ,\left(
x_{1},y_{1}\right)
=(-\mu X,-1/2)r_{31}, \\
\left( x_{2},y_{2}\right) &=&\left( C_{2}X,0\right)r_{31} \textrm{
and }\left( x_{3},y_{3}\right) =(-\mu X,1/2)r_{31},
\end{eqnarray}
where $C_{2}$ and $C_{4}$ are defined by equations (\ref{22a}) and
(\ref{22b}) respectively, while
\begin{equation}
X=\frac{\sqrt{\beta ^{2}-1/4}}{C_{4}+\mu }.
\end{equation}

Following the same procedure, as in the equal mass cases, we have
tried different mass ratios between 0 and 1 and all of them are
unstable and hence the configuration is linearly unstable to
perturbations. Details of all mass ratios are given in
 table (\ref{Table1})

\begin{table*}
  \begin{center}
  \caption{Triangular configuration of four-body problem with two bigger
masses making the base of the triangle}\label{Table1}


\begin{tabular}{|c||c||c|}\hline

$\mu $   &      Eigenvalues    & Remarks \\ \hline \hline 1 &
$\lambda _{1,2}=\pm 4.24$ and $\lambda _{3,4}=\pm 2.679i$ &
Linearly unstable \\ \hline 0.9 & $\lambda _{1,2}=\pm3.513$ and
$\lambda _{3,4}=\pm 2.77i$ & Linearly unstable \\ \hline
 0.8 &
$\lambda _{1,2}=\pm 3.23$ and $\lambda _{3,4}=\pm 2.672i$ & Linearly unstable \\
\hline
 0.7 & $\lambda _{1,2}=\pm 3.022$ and $\lambda _{3,4}=\pm 2.573i$ & Linearly unstable \\
\hline 0.6 & $\lambda _{1,2}=\pm 2.845\textrm{   and }\lambda
_{3,4}=\pm 2.482i$ & Linearly unstable \\ \hline 0.5 & $\lambda
_{1,2}=\pm 2.688\textrm{   and }\lambda _{3,4}=\pm 2.392i$ &
Linearly unstable \\ \hline 0.4 & $\lambda _{1,2}=\pm 2.54\textrm{
  and }\lambda _{3,4}=\pm 2.304i$ & Linearly
unstable \\ \hline 0.3 & $\lambda _{1,2}=\pm 2.52\textrm{
 and }\lambda _{3,4}=\pm 2.322i$ & Linearly unstable \\
\hline
 0.2 & $\lambda _{1,2}=\pm 2.24$ and $\lambda _{3,4}=\pm 2.11i$ & Linearly unstable \\
\hline
0.1 & $\lambda _{1,2}=\pm2.048$ and $\lambda _{3,4}=\pm 1.985i$ & Linearly unstable \\
\hline 0.0001 & $\lambda _{1,2}= \pm 2.039$ and $ \lambda
_{3,4}=\pm 1.98i$ & Linearly unstable
\\ \hline
$10^{-7}$ & $\lambda _{1,2}= \pm 1.51$ and $ \lambda _{3,4}= \pm
1.59i$ & Linearly unstable \\ \hline $10^{-10}$ & $\lambda
_{1,2}=\pm 1.46$ and $\lambda _{3,4}=\pm 1.558i$ & Linearly
unstable \\ \hline
\end{tabular}
 % }
\end{center}
\end{table*}
\subsection{The Triangular equilibrium configuration of the four-body problem with two smaller
masses making the base of the triangle}

Consider the triangular configuration of the four-body problem
having two pairs of two equal masses with the fourth mass on the
negative y-axis and the two smaller masses making the base of the
triangle. We have already obtained equilibrium solutions for it
and now will discuss its stability.

The initial conditions are
\begin{equation}
\left.
\begin{array}{c}
\left( x,y\right) =\left( \frac{1}{2}-\mu \alpha ,0\right)r
,\left( x_{1},y_{1}\right) =\left( \alpha ,\beta \right)r
,\textrm{ \ \ \ \ \ \ \ \ }
\\
\left( x_{2},y_{2}\right) =\left( -\frac{1}{2}-\mu \alpha
,0\right)r ,\left( x_{3},y_{3}\right) =\left( \alpha ,-\beta
\right)r
\end{array}
\right\}
\end{equation}
Following the same procedure, as in all other cases, we find that
all the equilibrium points are linearly unstable to perturbations.
For more details see table (\ref{Table2}).

\begin{table*}
  \begin{center}
  \caption{The Triangular configuration of four-body problem with two smaller
masses making the base of the triangle}\label{Table2}




\begin{tabular}{|c||c||c|}\hline

$\mu $ & Eigenvalues & Remarks\\ \hline \hline 1 & $\lambda =\pm
0.946 \pm 0.978i $ & Linearly unstable\\ \hline 0.999 & $\lambda =
\pm
0.94 \pm 0.981i $ & Linearly unstable \\
\hline 0.998 & $\lambda =\pm 0.93 \pm 0.983i $ & Linearly unstable
 \\ \hline 0.9975 & $\lambda
=\pm 0.904 \pm 0.99i $  & Linearly unstable  \\
\hline 0.9973 & $\lambda
=\pm 0.91\pm 0.991i $ & Linearly unstable  \\
\hline

\end{tabular}
 % }
\end{center}
\end{table*}


\subsection{The Trapezoidal Equilibrium Configuration with two pairs of equal
masses}

Consider the Trapezoidal equilibrium configurations of the four
body problem with two pairs of equal masses. Let the origin of the
coordinate system be the centre of mass of the system. The initial
positions of the three masses are the following:
\begin{eqnarray}
P_{1}(M) =(-1/2,-\frac{\mu \beta}{\mu +1})r, \nonumber \\
P_{2}(m)=(-\alpha /2,\frac{\beta}{\mu +1})r,\quad  \nonumber \\
P_{3}(m) =(\alpha /2,\frac{\beta}{\mu +1})r.,\qquad
\end{eqnarray}
The fourth mass, whose stability is under discussion, has an
initial position at $(1/2,-\frac{\mu \beta}{\mu +1})$. Here $\mu $
is the mass ratio and $\alpha ,\beta $ are the distance ratios.
All three ratios are related to each other by two highly
non-linear algebraic equations, given in chapter 2. Like others,
the equilibrium points for this configuration are also given in
chapter 2 \cite{RoyandSteves1998}.

For the mass ratio equal to one this becomes a special case of the
equal mass four body problem i.e. Equilibrium Configuration of
four body problem with four equal masses making a square, which is
an unstable equilibrium configuration discussed before. Other mass
ratios between 0 and 1 have also been analyzed and all of them
turned out to be linearly unstable. For further details on other
mass ratios see table 3.3.

\begin{table*}
  \begin{center}
  \caption{Trapezoidal Equilibrium Configuration with two pairs of equal
masses}\label{Table3}

\bigskip

\begin{tabular}{|c||c||c|}\hline

$\mu $ & Eigenvalues & Remarks \\ \hline \hline

1 & Indeterminate & Linearly unstable \\ \hline 0.9 & $\lambda
_{1,2}=\pm (86.26i)$ and $\lambda _{3,4}=\pm 110.549$ & Linearly unstable \\
\hline 0.8 & $\lambda _{1,2}=\pm (28.26i)$
 and $\lambda _{3,4}=\pm 36.137$ & Linearly unstable \\
\hline .7 & $\lambda _{1,2}=\pm (14.202i)$  and $\lambda
_{3,4}=\pm 17.986$ & Linearly unstable \\ \hline .6 & $\lambda
_{1,2}=\pm (8.45i)$  and $\lambda _{3,4}=\pm 10.57$ & Linearly
unstable \\ \hline .5 & $\lambda _{1,2}=\pm (5.5i)$
 and $\lambda _{3,4}=\pm 6.734$ & Linearly unstable \\
\hline .4 & $\lambda _{1,2}=\pm (3.76i)$   and $\lambda _{3,4}=\pm
4.41$ & Linearly unstable \\ \hline .3 & $\lambda _{1,2}=\pm
(2.65i)$  and $\lambda _{3,4}=\pm 2.83$ & Linearly unstable \\
\hline .2 & $\lambda _{1,2}=\pm (1.81i)$
 and $\lambda _{3,4}=\pm 2.02$ & Linearly unstable \\
\hline .1 & $\lambda _{1,2}=\pm (1.92i)$  and $\lambda _{3,4}=\pm
1.46$ & Linearly unstable \\ \hline
\end{tabular}

 % }
\end{center}
\end{table*}

\subsection{The Diamond Equilibrium Configuration with two pairs of equal masses}

We discuss here the stability of the diamond equilibrium
configuration of the four body problem, with two pairs of equal
masses. This is a highly symmetric, being symmetric about both the
x-axis and the y-axis. The origin of the coordinate system is the
centre of mass of the system under discussion. The initial
positions of the three masses are the following:
\begin{equation}
P_{1}(M)=(-1,0)r,P_{2}(m)=(0,\alpha )r\textrm{ and
}P_{3}(m)=(1,0)r,
\end{equation}
The fourth mass, whose stability is under discussion, has its
initial position at $(0,-\alpha )$. Here $\mu $ is the mass ratio
and $\alpha $ is the distance ratio. We used the same method for
stability analysis of this configuration as we have used for
others. The stability for different mass ratios is was analyzed
and all of them turn out to be linearly unstable to perturbations.
Results obtained for the different mass ratios are shown in table
(\ref{Table4})

\begin{table*}
  \begin{center}
  \caption{Diamond Equilibrium Configuration with two pairs of equal masses}\label{Table4}

\bigskip

\begin{tabular}{|c||c||c|}\hline
$\mu $ & Eigenvalues & Remarks \\ \hline \hline 1 & $\lambda
_{1,2}=\pm (0.409-0.86i)$ and $ \lambda _{3,4}=\pm (0.409+0.86i)$
& Linearly unstable \\ \hline .9 & $\lambda _{1,2}=\pm (0.4-0.9i)$
and\ $\lambda _{3,4}=\pm (0.4+0.9i)$ & Linearly unstable
\\ \hline .8 & $\lambda _{1,2}=\pm (0.39-0.91i)$  and
$\lambda _{3,4}=\pm (0.39+0.91i)$ & Linearly unstable \\ \hline .7
& $\lambda _{1,2}=\pm (0.38-0.93i)$  and $\lambda _{3,4}=\pm
(0.38+0.93i)$ & Linearly unstable \\ \hline .6 & $\lambda
_{1,2}=\pm (0.37-0.94i)$  and $\lambda _{3,4}=\pm (0.37+0.94i)$ &
Linearly unstable \\ \hline .5 & $\lambda _{1,2}=\pm (0.36-0.95i)$
 and $\lambda _{3,4}=\pm (0.36+0.95i)$ & Linearly unstable
\\ \hline .4 & $\lambda _{1,2}=\pm (0.35-0.96i)$  and
$\lambda _{3,4}=\pm (0.35+0.96i)$ & Linearly unstable \\ \hline .3
& $\lambda _{1,2}=\pm (0.34-0.97i) $ and $\lambda _{3,4}=\pm
(0.34+0.97i)$ & Linearly unstable \\ \hline .2 & $\lambda
_{1,2}=\pm (0.33-0.98i)$  and $\lambda _{3,4}=\pm (0.33+0.98i)$ &
Linearly unstable \\ \hline .1 & $\lambda _{1,2}=\pm (0.32-0.98i)
$ and $\lambda _{3,4}=\pm (0.32+0.98i)$ & Linearly unstable \\
\hline 0 & $\lambda _{1,2}=\pm (0.3-0.98i)$ and $\lambda
_{3,4}=\pm (0.3+0.98i)$ & Linearly unstable
\\ \hline
\end{tabular}

 % }
\end{center}
\end{table*}

\subsection{Collinear Equilibrium Configurations with two pairs of equal mass
}

\subsubsection{Case-I}

Consider the collinear equilibrium configuration of the four-body
problem having two pairs of equal masses with the smaller masses
at the ends of the line while the larger masses lie in the middle.
We will discuss the linear stability of the equilibrium solutions
obtained in chapter 2.

The initial conditions for all mass ratios in this case are
\begin{equation}
{\bf r}_{1}=(1,0)r,\textrm{ }{\bf r}_{2}=\left( \alpha ,0\right)r
,\textrm{ }{\bf r }_{3}=\left( -\alpha ,0\right)r ,\textrm{ and
}\left( x,y\right) =\left( -1,0\right)r ,
\end{equation}
where $\alpha $ has different value for different values of $\mu
.$
\begin{equation}
U_{xx}=1+2A,U_{yy}=1-A\textrm{ and }U_{xy}=0,
\end{equation}
where
\begin{equation}
A=\frac{m}{r_{1}^{3}}+\frac{M}{r_{2}^{3}}+\frac{M}{r_{3}^{3}}.
\label{A}
\end{equation}
Hence the characteristic equation becomes
\begin{equation}
\lambda ^{4}+\left( 2-A\right) \lambda ^{2}+\left(
1+A-2A^{2}\right) =0. \label{ChEq}
\end{equation}
The eigenvalues becomes
\begin{equation}
\lambda _{1,2}=\pm i\sqrt{2\left( 1+A\right) }\textrm{ and }\lambda _{3,4}=%
\sqrt{2\left( 2A-1\right) }.  \label{case-1}
\end{equation}
In order to have stable equilibrium points all the eigenvalues
should be pure imaginary. Therefore we must establish if $\lambda
_{3,4}$ is real or imaginary. As $A$ always remain greater than 1,
 $\lambda _{3,4}$ is always a real number. Thus the
equilibrium configuration is linearly unstable for all values of
the mass ratio $\mu .$

\subsubsection{Case-II}

Consider the collinear equilibrium configuration of the four-body
problem having two pairs of equal masses with the larger masses at
the ends of the line while the smaller masses lie in the middle.
We will discuss the linear stability of the equilibrium solutions
obtained in chapter 2.

The initial conditions remain the same as for case-I and therefore
the form of eigenvalues also remain the same as given in
(\ref{case-1}). The value of $A$ remains greater than 1 for all
values of the mass ratio $\mu $ and thus $\lambda _{3,4}$ is real
and the equilibrium configurations are unstable.

\subsubsection{Cases-III and IV}

Consider the non-symmetric collinear equilibrium configuration of
the four-body problem with two pairs of equal masses having
smaller and bigger masses alternatively on the straight line.

The initial conditions are
\begin{equation}
{\bf r}_{1}=(1,0)r,\textrm{ }{\bf r}_{2}=\left( \alpha ,0\right)r
,\textrm{ }{\bf r }_{3}=\left( -\beta ,0\right)r ,\textrm{ and
}\left( x,y\right) =\left( -\gamma ,0\right)r ,
\end{equation}
where $\alpha ,\beta $ and $\gamma $ are the distance ratios
having different values for different values of $\mu$. All these
ratios satisfy the following expression
\begin{equation}
\gamma =\alpha +\mu \left( 1-\beta \right) .
\end{equation}
The characteristic equation and therefore the form of the
eigenvalues remain the same as in the first case and are given by
(\ref{ChEq}) and (\ref{case-1} ). After careful inspection of
(\ref{A}), we conclude that it remains greater than 1 for all
values of $\mu $ and therefore $\lambda _{3,4}$ is real. Hence
this equilibrium configuration is also unstable to perturbations.
Similarly the fourth and final collinear equilibrium configuration
(discussed in chapter 2) turns out to be unstable.

\section{Summary and conclusions}

We discuss the linear stability of equilibrium solutions of the
four body problems which included equal mass problem
\cite{RoyandSteves1998} and those with two pairs of equal masses.

We have extended the method given by \citeasnoun{CarlMurray} for
the three body problem, to the general four body problem. We
applied this method to all the equilibrium solutions we have
determined for the four body problem in chapter 3. All these
solutions are unstable to perturbations. Therefore it is unlikely
that such four body stellar systems would exist for a substantial
period of time and hence they are unlikely to be observed in these
configurations.

